Extreme & High Synchrotron Peaked Blazars at the limit of Fermi-LAT detectability: the $\gamma$-ray spectrum of 1BIGB sources

We present the 1-100 GeV spectral energy distribution for a population of 148 high-synchrotron-peaked blazars (HSPs) recently detected with Fermi-LAT as part of the First Brazil-ICRANet Gamma-ray Blazar catalogue (1BIGB). Most of the 1BIGB sources do not appear in previous Fermi-LAT catalogues and their gamma-ray spectral properties are presented here for the first time, representing a significant new extension of the gamma-ray blazar population. Since our sample was originally selected from an excess signal in the 0.3-500 GeV band, the sources stand out as promising TeV blazar candidates, potentially in reach of the forthcoming very-high-energy (VHE) gamma-ray observatory, CTA. The flux estimates presented here are derived considering PASS8 data, integrating over more than 9 years of Fermi-LAT observations. We also review the full broadband fit between 0.3-500 GeV presented in the original 1BIGB paper for all sources, updating the power-law parameters with currently available Fermi-LAT dataset. The importance of these sources in the context of VHE population studies with both current instruments and the future CTA is evaluated. To do so, we select a subsample of 1BIGB sources and extrapolate their gamma-ray SEDs to the highest energies, properly accounting for absorption due to the extragalactic background light. We compare those extrapolations to the published CTA sensitivity curves and estimate their detectability by CTA. Two notable sources from our sample, namely 1BIGB J224910.6-130002 and 1BIGB J194356.2+211821, are discussed in greater detail. All gamma-ray SEDs, which are shown here for the first time, are made publicly available via the Brazilian Science Data Center (BSDC) service, maintained at CBPF, in Rio de Janeiro.

==> arXiv-1BIGB-9yrs-long-table.tex <==
%LONG-TABLE-1
\begin{table*}
\caption{Table showing the 148 1BIGB $\gamma$-ray signatures. The first three columns show respectively the 1BIGB source names, right ascension R.A. and declination Dec. in degrees (J2000). The fourth column shows the reported redshifts from literature \citep{bllacz2,pita2013,pks1424p240HighZ,PG1553,shaw2,masetti2013,bll,5BZcat},  flag ? is used for values reported as uncertain; lower limit are marked with ``$>$" \citep[all lower-limits shown here were derived in][]{1WHSP,2WHSP}, and sources with currently absent redshift were given 0. value. The $\gamma$-ray model parameters from Fermi Science Tools assume a power law to describe the spectrum within the studied energy range 0.3-500 GeV. The parameter $N_0$ (see eq. \ref{powerlaw}) is given in units of [ph/cm$^{2}$/s/MeV], and $\Gamma$ is the spectral photon index, which are direct outputs from the likelihood analysis over 7.2 years of Fermi-LAT data in the 0.3-500\,GeV band; those results consider the pivot energy fixed as E$_0$\,=\,1\,GeV. The column Flux gives the photon counts in units of ph/cm$^2$/s calculated by integrating eq. \ref{powerlaw} along the energy range 1-100\,GeV, column E-FLux corresponds to the energy flux in units of MeV/cm$^2$/s. For the columns Flux and E-flux, upper and lower case values represent positive and negative errors, respectively.}
\label{table:1BIGB}
 \begin{tabular}{llrcccccc}
\hline
1BIGB Source name  & R.A.(deg)  &  Dec.(deg)  &  z  &  $\Gamma$ & $N_0$ (10$^{-15}$)  & TS & Flux$_{1-100GeV}^{( \times 10^{-10})}$ & E-Flux$_{1-100GeV}^{( \times 10^{-13})}$ \\
 \hline
  1BIGBJ000949.6-431650  &   2.45708    &   -43.28056  &  $>$0.56    &  2.19$\pm$0.13  &   2.29$\pm$0.40   &   86.2 &  1.92$^{+0.63}_{-0.50}$   &  7.0$^{+2.3}_{-1.5}$ \\ 
  1BIGBJ001328.8+094929  &   3.37       &   9.825      &     0.      &  2.07$\pm$0.19  &   1.56$\pm$0.57   &   24.6 &  1.44$^{+0.95}_{-0.67}$   &  6.0$^{+3.5}_{-1.9}$ \\ 
  1BIGBJ001527.8+353638  &   3.86625    &   35.61083   &  $>$0.57    &  1.90$\pm$0.23  &   0.94$\pm$0.48   &   35.3 &  1.02$^{+0.99}_{-0.62}$   &  5.4$^{+4.7}_{-2.2}$ \\ 
  1BIGBJ002928.6+205332  &   7.36917    &   20.8925    &     0.      &  1.66$\pm$0.19  &   0.59$\pm$0.31   &   29.5 &  0.85$^{+0.87}_{-0.53}$   &  6.5$^{+5.3}_{-2.7}$ \\ 
  1BIGBJ004146.9-470136  &   10.44583   &   -47.02667  &     0.      &  1.79$\pm$0.27  &   0.33$\pm$0.21   &   10.8 &  0.40$^{+0.55}_{-0.30}$   &  2.5$^{+3.0}_{-1.2}$ \\ 
  1BIGBJ005816.6+172312  &   14.56958   &   17.38694   &     0.      &  1.79$\pm$0.24  &   0.73$\pm$0.44   &   24.0 &  0.89$^{+1.07}_{-0.62}$   &  5.6$^{+5.7}_{-2.5}$ \\ 
  1BIGBJ010250.8-200158  &   15.71208   &   -20.03278  &  $>$0.38    &  1.49$\pm$0.23  &   0.25$\pm$0.17   &   20.4 &  0.45$^{+0.68}_{-0.35}$   &  4.6$^{+5.2}_{-2.2}$ \\ 
  1BIGBJ011501.6-340027  &   18.75708   &   -34.0075   &     0.48    &  1.65$\pm$0.16  &   0.82$\pm$0.36   &   70.8 &  1.19$^{+0.98}_{-0.64}$   &  9.2$^{+6.1}_{-3.4}$ \\ 
  1BIGBJ012657.1+330730  &   21.73833   &   33.125     &     0.      &  2.19$\pm$0.29  &   1.38$\pm$0.57   &   22.2 &  1.15$^{+0.99}_{-0.61}$   &  4.2$^{+3.9}_{-1.6}$ \\ 
  1BIGBJ014040.8-075849  &   25.17      &   -7.98028   &  $>$0.49    &  1.77$\pm$0.14  &   1.12$\pm$0.37   &   45.0 &  1.41$^{+0.85}_{-0.61}$   &  9.1$^{+4.7}_{-2.9}$ \\ 
  1BIGBJ020106.1+003400  &   30.27542   &   0.56667    &     0.298   &  1.70$\pm$0.24  &   0.47$\pm$0.30   &   19.9 &  0.65$^{+0.84}_{-0.47}$   &  4.7$^{+5.0}_{-2.2}$ \\ 
  1BIGBJ020412.9-333339  &   31.05375   &   -33.56111  &     0.617   &  1.85$\pm$0.19  &   0.87$\pm$0.35   &   31.7 &  1.00$^{+0.78}_{-0.51}$   &  5.7$^{+4.1}_{-2.1}$ \\ 
  1BIGBJ021205.6-255757  &   33.02375   &   -25.96611  &     0.      &  1.99$\pm$0.14  &   1.67$\pm$0.41   &   58.9 &  1.67$^{+0.74}_{-0.56}$   &  7.8$^{+3.3}_{-2.1}$ \\ 
  1BIGBJ021216.8-022155  &   33.07      &   -2.36528   &     0.      &  1.92$\pm$0.19  &   1.16$\pm$0.44   &   31.8 &  1.23$^{+0.89}_{-0.60}$   &  6.3$^{+4.3}_{-2.3}$ \\ 
  1BIGBJ021631.9+231449  &   34.13333   &   23.24722   &     0.288   &  1.88$\pm$0.10  &   2.49$\pm$0.52   &  116.4 &  2.76$^{+0.98}_{-0.79}$   & 15.0$^{+4.7}_{-3.3}$ \\ 
  1BIGBJ022048.4-084250  &   35.20167   &   -8.71389   &  $>$0.43    &  1.88$\pm$0.20  &   1.00$\pm$0.43   &   34.1 &  1.11$^{+0.90}_{-0.59}$   &  6.0$^{+4.3}_{-2.2}$ \\ 
  1BIGBJ023340.9+065611  &   38.42042   &   6.93639    &     0.      &  2.03$\pm$0.14  &   3.23$\pm$0.90   &   98.0 &  3.08$^{+1.45}_{-1.12}$   & 13.6$^{+5.4}_{-3.5}$ \\ 
  1BIGBJ023430.5+804336  &   38.6275    &   80.72694   &     0.      &  1.55$\pm$0.14  &   0.37$\pm$0.16   &   32.4 &  0.63$^{+0.49}_{-0.34}$   &  5.8$^{+3.2}_{-1.9}$ \\ 
  1BIGBJ030103.7+344100  &   45.26542   &   34.68361   &     0.24    &  2.33$\pm$0.16  &   3.26$\pm$0.63   &   56.3 &  2.43$^{+0.87}_{-0.68}$   &  7.6$^{+2.7}_{-1.7}$ \\ 
  1BIGBJ030330.1+055429  &   45.87542   &   5.90833    &     0.196   &  1.50$\pm$0.23  &   0.33$\pm$0.26   &   24.5 &  0.60$^{+0.99}_{-0.51}$   &  6.0$^{+7.0}_{-3.0}$ \\ 
  1BIGBJ030433.9-005403  &   46.14125   &   -0.90111   &     0.511   &  1.69$\pm$0.16  &   0.79$\pm$0.35   &   38.1 &  1.09$^{+0.87}_{-0.59}$   &  7.9$^{+5.0}_{-2.8}$ \\ 
  1BIGBJ030544.1+403509  &   46.43375   &   40.58611   &     0.      &  1.88$\pm$0.25  &   0.77$\pm$0.46   &   19.0 &  0.85$^{+0.98}_{-0.58}$   &  4.6$^{+4.5}_{-2.0}$ \\ 
  1BIGBJ031103.1-440227  &   47.76333   &   -44.04111  &     0.      &  1.96$\pm$0.35  &   0.72$\pm$0.43   &   16.4 &  0.73$^{+1.03}_{-0.52}$   &  3.5$^{+5.5}_{-1.8}$ \\ 
  1BIGBJ031423.8+061955  &   48.59958   &   6.33222    &     0.62?   &  1.78$\pm$0.11  &   2.25$\pm$0.58   &   92.4 &  2.78$^{+1.22}_{-0.95}$   & 17.6$^{+6.4}_{-4.4}$ \\ 
  1BIGBJ032009.1-704533  &   50.03833   &   -70.75917  &     0.      &  1.77$\pm$0.18  &   0.63$\pm$0.26   &   32.1 &  0.79$^{+0.63}_{-0.41}$   &  5.1$^{+3.5}_{-1.9}$ \\ 
  1BIGBJ032037.9+112451  &   50.15833   &   11.41444   &     0.      &  2.36$\pm$0.24  &   3.12$\pm$0.99   &   24.8 &  2.27$^{+1.35}_{-0.95}$   &  6.9$^{+3.9}_{-2.1}$ \\ 
  1BIGBJ032056.2+042447  &   50.23458   &   4.41333    &     0.      &  2.70$\pm$0.22  &   3.03$\pm$0.61   &   30.1 &  1.78$^{+0.69}_{-0.52}$   &  4.1$^{+1.5}_{-0.9}$ \\ 
  1BIGBJ032647.2-340446  &   51.69708   &   -34.07972  &     0.      &  2.04$\pm$0.12  &   1.96$\pm$0.38   &   76.7 &  1.86$^{+0.64}_{-0.51}$   &  8.1$^{+2.7}_{-1.8}$ \\ 
  1BIGBJ032852.6-571605  &   52.21917   &   -57.26806  &     0.      &  1.55$\pm$0.18  &   0.36$\pm$0.19   &   36.3 &  0.61$^{+0.65}_{-0.39}$   &  5.6$^{+4.6}_{-2.4}$ \\ 
  1BIGBJ033623.7-034738  &   54.09875   &   -3.79389   &     0.162   &  1.44$\pm$0.19  &   0.36$\pm$0.23   &   41.6 &  0.71$^{+0.93}_{-0.52}$   &  7.8$^{+7.1}_{-3.5}$ \\ 
  1BIGBJ033831.9-570447  &   54.63333   &   -57.08     &     0.      &  1.89$\pm$0.27  &   0.43$\pm$0.25   &   10.6 &  0.48$^{+0.56}_{-0.32}$   &  2.5$^{+2.8}_{-1.1}$ \\ 
  1BIGBJ035856.1-305447  &   59.73375   &   -30.91306  &     0.65?   &  1.92$\pm$0.14  &   1.43$\pm$0.40   &   59.6 &  1.53$^{+0.76}_{-0.57}$   &  7.9$^{+3.6}_{-2.2}$ \\ 
  1BIGBJ041112.2-394143  &   62.80125   &   -39.69528  &  $>$0.7     &  1.74$\pm$0.29  &   0.23$\pm$0.19   &    6.7 &  0.31$^{+0.53}_{-0.26}$   &  2.1$^{+3.0}_{-1.1}$ \\ 
  1BIGBJ041238.3-392629  &   63.16      &   -39.44139  &     0.      &  1.91$\pm$0.30  &   0.34$\pm$0.25   &    6.7 &  0.37$^{+0.54}_{-0.29}$   &  1.9$^{+2.5}_{-9.5}$ \\ 
  1BIGBJ042900.1-323641  &   67.25042   &   -32.61139  &  $>$0.51    &  2.04$\pm$0.17  &   1.20$\pm$0.36   &   27.9 &  1.13$^{+0.63}_{-0.45}$   &  4.9$^{+2.6}_{-1.5}$ \\ 
  1BIGBJ043517.7-262121  &   68.82375   &   -26.35611  &     0.      &  2.60$\pm$0.28  &   1.64$\pm$0.43   &   20.2 &  1.02$^{+0.54}_{-0.38}$   &  2.5$^{+1.4}_{-0.7}$ \\ 
  1BIGBJ044127.4+150454  &   70.36417   &   15.08194   &     0.109   &  2.10$\pm$0.18  &   3.03$\pm$1.18   &   43.0 &  2.74$^{+1.81}_{-1.30}$   & 11.1$^{+6.0}_{-3.4}$ \\ 
  1BIGBJ044240.6+614039  &   70.66917   &   61.6775    &     0.      &  2.01$\pm$0.09  &   4.00$\pm$0.71   &  145.0 &  3.92$^{+1.12}_{-0.95}$   & 17.9$^{+4.3}_{-3.2}$ \\ 
  1BIGBJ044328.3-415156  &   70.86833   &   -41.86556  &  $>$0.39    &  1.96$\pm$0.15  &   1.58$\pm$0.44   &   66.8 &  1.63$^{+0.83}_{-0.61}$   &  8.0$^{+3.8}_{-2.3}$ \\ 
  1BIGBJ050335.3-111506  &   75.8975    &   -11.25167  &  $>$0.57    &  1.85$\pm$0.11  &   2.30$\pm$0.53   &  102.6 &  2.63$^{+1.03}_{-0.82}$   & 15.0$^{+5.1}_{-3.5}$ \\ 
  1BIGBJ050419.5-095631  &   76.08125   &   -9.94222   &  $>$0.46    &  2.14$\pm$0.23  &   1.29$\pm$0.54   &   16.6 &  1.12$^{+0.86}_{-0.58}$   &  4.3$^{+3.0}_{-1.5}$ \\ 
  1BIGBJ050601.6-382054  &   76.50667   &   -38.34861  &     0.182   &  1.95$\pm$0.11  &   2.06$\pm$0.40   &   96.5 &  2.13$^{+0.73}_{-0.59}$   & 10.5$^{+3.4}_{-2.4}$ \\ 
  1BIGBJ050727.1-334635  &   76.86333   &   -33.77639  &     0.      &  1.79$\pm$0.11  &   1.84$\pm$0.43   &  125.0 &  2.25$^{+0.93}_{-0.72}$   & 14.1$^{+5.0}_{-3.5}$ \\ 
  1BIGBJ053626.8-254748  &   84.11167   &   -25.79667  &     0.      &  2.06$\pm$0.16  &   1.70$\pm$0.44   &   47.9 &  1.58$^{+0.76}_{-0.56}$   &  6.7$^{+3.1}_{-1.9}$ \\ 
  1BIGBJ053645.2-255841  &   84.18875   &   -25.97806  &     0.      &  1.92$\pm$0.18  &   1.20$\pm$0.44   &   33.8 &  1.28$^{+0.88}_{-0.60}$   &  6.6$^{+4.2}_{-2.3}$ \\ 
  1BIGBJ055716.7-061706  &   89.32      &   -6.285     &     0.      &  1.95$\pm$0.15  &   2.51$\pm$0.86   &   52.2 &  2.59$^{+1.52}_{-1.12}$   & 12.7$^{+6.3}_{-3.8}$ \\ 
  1BIGBJ060714.2-251859  &   91.80958   &   -25.31639  &     0.275   &  1.94$\pm$0.14  &   1.54$\pm$0.40   &   51.9 &  1.61$^{+0.75}_{-0.57}$   &  8.1$^{+3.4}_{-2.2}$ \\ 
  1BIGBJ062149.6-341148  &   95.45667   &   -34.19694  &     0.529   &  2.53$\pm$0.12  &   4.77$\pm$0.59   &   93.3 &  3.09$^{+0.68}_{-0.58}$   &  8.1$^{+1.6}_{-1.2}$ \\ 
  1BIGBJ062626.2-171045  &   96.60917   &   -17.17944  &  $>$0.7     &  2.00$\pm$0.18  &   1.80$\pm$0.66   &   34.6 &  1.78$^{+1.17}_{-0.82}$   &  8.2$^{+4.9}_{-2.7}$ \\ 
  1BIGBJ063014.9-201236  &   97.5625    &   -20.21     &     0.      &  1.56$\pm$0.33  &   0.37$\pm$0.47   &   16.2 &  0.62$^{+1.79}_{-0.72}$   &  5.6$^{+11.0}_{-3.3}$ \\ 
  1BIGBJ065932.8-674350  &   104.88708  &   -67.73056  &     0.      &  1.63$\pm$0.17  &   0.55$\pm$0.29   &   39.4 &  0.82$^{+0.78}_{-0.50}$   &  6.5$^{+4.6}_{-2.5}$ \\ 
 1BIGBJ071745.0-552021  &   109.4375   &   -55.33944  &     0.      &  2.12$\pm$0.14  &   2.32$\pm$0.53   &   60.9 &  2.05$^{+0.83}_{-0.65}$   &  8.1$^{+3.0}_{-2.0}$ \\ 
  1BIGBJ073152.6+280432  &   112.96958  &   28.07583   &     0.248   &  1.90$\pm$0.18  &   1.06$\pm$0.39   &   29.9 &  1.15$^{+0.79}_{-0.54}$   &  6.1$^{+3.8}_{-2.1}$ \\ 
  1BIGBJ073329.5+351542  &   113.37292  &   35.26167   &     0.177   &  2.56$\pm$0.23  &   1.71$\pm$0.42   &   21.0 &  1.09$^{+0.51}_{-0.37}$   &  2.8$^{+1.2}_{-0.7}$ \\  
  1BIGBJ075936.1+132116  &   119.90042  &   13.35472   &     0.      &  1.75$\pm$0.09  &   2.12$\pm$0.44   &  152.6 &  2.71$^{+0.98}_{-0.79}$   & 17.9$^{+5.5}_{-4.0}$ \\ 
  1BIGBJ080015.4+561107  &   120.06458  &   56.18528   &     0.      &  1.92$\pm$0.12  &   1.54$\pm$0.34   &   78.9 &  1.65$^{+0.65}_{-0.51}$   &  8.5$^{+3.1}_{-2.1}$ \\ 
  1BIGBJ082904.7+175415  &   127.27     &   17.90417   &     0.089   &  2.25$\pm$0.10  &   4.47$\pm$0.55   &  136.8 &  3.55$^{+0.79}_{-0.67}$   & 12.1$^{+2.7}_{-2.0}$ \\ 
  1BIGBJ083724.5+145819  &   129.3525   &   14.97222   &     0.278   &  1.75$\pm$0.15  &   1.07$\pm$0.37   &   50.6 &  1.37$^{+0.87}_{-0.61}$   &  9.1$^{+4.9}_{-2.9}$ \\ 
  1BIGBJ085749.8+013530  &   134.4575   &   1.59167    &     0.281   &  2.57$\pm$0.23  &   1.81$\pm$0.48   &   18.6 &  1.15$^{+0.56}_{-0.42}$   &  2.9$^{+1.3}_{-0.7}$ \\  
  1BIGBJ090802.2-095936  &   137.00917  &   -9.99361   &     0.053   &  1.79$\pm$0.26  &   0.68$\pm$0.49   &   22.5 &  0.83$^{+1.17}_{-0.65}$   &  5.2$^{+5.8}_{-2.4}$ \\ 
  1BIGBJ090953.2+310602  &   137.47167  &   31.10083   &     0.272   &  1.81$\pm$0.21  &   0.62$\pm$0.32   &   22.3 &  0.75$^{+0.73}_{-0.45}$   &  4.5$^{+3.7}_{-1.8}$ \\ 
  1BIGBJ091322.3+813305  &   138.34292  &   81.55139   &     0.639?  &  1.40$\pm$0.15  &   0.20$\pm$0.10   &   41.5 &  0.42$^{+0.42}_{-0.26}$   &  4.9$^{+3.4}_{-1.9}$ \\ 
  1BIGBJ091651.8+523827  &   139.21625  &   52.64111   &     0.19    &  1.97$\pm$0.17  &   1.17$\pm$0.35   &   60.6 &  1.18$^{+0.67}_{-0.48}$   &  5.7$^{+3.1}_{-1.8}$ \\ 
  1BIGBJ093239.2+104234  &   143.16375  &   10.70972   &     0.361   &  2.00$\pm$0.14  &   1.95$\pm$0.49   &   58.5 &  1.92$^{+0.87}_{-0.66}$   &  8.9$^{+3.7}_{-2.4}$ \\ 
  1BIGBJ093430.1-172120  &   143.62542  &   -17.35583  &     0.      &  1.75$\pm$0.22  &   0.79$\pm$0.50   &   20.9 &  1.02$^{+1.22}_{-0.72}$   &  6.7$^{+6.4}_{-2.9}$ \\ 
  1BIGBJ095224.1+750212  &   148.10042  &   75.03694   &     0.181   &  1.43$\pm$0.15  &   0.29$\pm$0.14   &   62.4 &  0.57$^{+0.54}_{-0.34}$   &  6.3$^{+4.2}_{-2.4}$ \\ 
  1BIGBJ095507.9+355100  &   148.78292  &   35.85      &     0.834   &  2.00$\pm$0.25  &   0.82$\pm$0.38   &   24.1 &  0.80$^{+0.74}_{-0.46}$   &  3.7$^{+3.3}_{-1.5}$ \\ 
  1BIGBJ095628.2-095719  &   149.1175   &   -9.95528   &     0.      &  1.80$\pm$0.26  &   0.60$\pm$0.40   &   16.1 &  0.73$^{+0.98}_{-0.54}$   &  4.5$^{+5.2}_{-2.1}$ \\ 
  1BIGBJ095849.8+703959  &   149.7075   &   70.66639   &     0.      &  1.98$\pm$0.23  &   0.99$\pm$0.43   &   37.1 &  0.99$^{+0.84}_{-0.54}$   &  4.7$^{+3.7}_{-1.8}$ \\ 
  1BIGBJ102100.3+162554  &   155.25125  &   16.43167   &     0.556   &  2.16$\pm$0.23  &   1.48$\pm$0.52   &   27.9 &  1.27$^{+0.86}_{-0.58}$   &  4.8$^{+3.2}_{-1.6}$ \\ 
  1BIGBJ104303.7+005420  &   160.76583  &   0.90556    &     0.      &  1.75$\pm$0.14  &   1.30$\pm$0.43   &   56.5 &  1.67$^{+1.00}_{-0.72}$   & 11.0$^{+5.5}_{-3.4}$ \\ 
  1BIGBJ104857.6+500945  &   162.24     &   50.1625    &     0.402   &  2.37$\pm$0.15  &   2.01$\pm$0.35   &   53.1 &  1.46$^{+0.47}_{-0.38}$   &  4.4$^{+1.4}_{-0.9}$ \\ 
  1BIGBJ105534.3-012616  &   163.89292  &   -1.43778   &     0.      &  1.66$\pm$0.11  &   1.53$\pm$0.43   &   99.0 &  2.20$^{+1.08}_{-0.82}$   & 16.9$^{+6.6}_{-4.5}$ \\ 
  1BIGBJ111717.5+000633  &   169.32292  &   0.10917    &     0.451   &  1.92$\pm$0.15  &   1.87$\pm$0.53   &   57.4 &  2.00$^{+1.04}_{-0.76}$   & 10.3$^{+4.9}_{-3.0}$ \\ 
  1BIGBJ112317.9-323217  &   170.825    &   -32.53833  &     0.      &  2.06$\pm$0.22  &   1.25$\pm$0.48   &   22.8 &  1.16$^{+0.85}_{-0.57}$   &  4.9$^{+3.5}_{-1.7}$ \\ 
  1BIGBJ112611.8-203723  &   171.54958  &   -20.62333  &     0.      &  2.12$\pm$0.27  &   1.15$\pm$0.59   &   11.6 &  1.02$^{+0.99}_{-0.62}$   &  4.0$^{+3.5}_{-1.6}$ \\ 
  1BIGBJ113046.0-313807  &   172.69208  &   -31.63528  &     0.151   &  1.29$\pm$0.20  &   0.13$\pm$0.10   &   24.8 &  0.33$^{+0.56}_{-0.28}$   &  4.7$^{+5.0}_{-2.3}$ \\ 
  1BIGBJ113105.2-094405  &   172.77167  &   -9.735     &     0.      &  1.66$\pm$0.14  &   0.99$\pm$0.35   &   64.1 &  1.43$^{+0.92}_{-0.65}$   & 10.9$^{+5.7}_{-3.5}$ \\ 
  1BIGBJ113444.6-172900  &   173.68625  &   -17.48361  &     0.571   &  1.68$\pm$0.17  &   0.79$\pm$0.35   &   36.9 &  1.10$^{+0.91}_{-0.60}$   &  8.2$^{+5.4}_{-3.0}$ \\ 
  1BIGBJ113755.6-171041  &   174.48167  &   -17.17833  &     0.6     &  1.71$\pm$0.10  &   1.90$\pm$0.43   &  126.9 &  2.55$^{+1.00}_{-0.79}$   & 18.0$^{+6.0}_{-4.2}$ \\ 
  1BIGBJ121158.6+224233  &   182.99417  &   22.70917   &     0.45    &  1.83$\pm$0.17  &   0.89$\pm$0.34   &   30.2 &  1.04$^{+0.74}_{-0.50}$   &  6.0$^{+3.8}_{-2.1}$ \\ 
  1BIGBJ121510.9+073203  &   183.79542  &   7.53444    &     0.137   &  1.64$\pm$0.11  &   1.26$\pm$0.37   &  105.5 &  1.87$^{+0.97}_{-0.72}$   & 14.9$^{+6.2}_{-4.1}$ \\ 
  1BIGBJ121603.1-024304  &   184.01333  &   -2.71778   &     0.169   &  2.22$\pm$0.16  &   2.81$\pm$0.67   &   56.3 &  2.28$^{+0.97}_{-0.74}$   &  8.0$^{+3.2}_{-2.0}$ \\ 
  1BIGBJ124141.4+344029  &   190.4225   &   34.675     &  $>$0.7     &  1.88$\pm$0.15  &   1.19$\pm$0.37   &   46.8 &  1.33$^{+0.76}_{-0.55}$   &  7.3$^{+3.8}_{-2.3}$ \\ 
  1BIGBJ125015.4+315559  &   192.56458  &   31.93306   &     0.      &  1.82$\pm$0.31  &   0.55$\pm$0.39   &   16.8 &  0.65$^{+1.02}_{-0.51}$   &  3.9$^{+5.7}_{-2.0}$ \\ 
  1BIGBJ125341.2-393159  &   193.42167  &   -39.53306  &     0.179   &  1.89$\pm$0.17  &   1.29$\pm$0.51   &   39.8 &  1.42$^{+1.00}_{-0.69}$   &  7.6$^{+4.6}_{-2.6}$ \\ 
  1BIGBJ125847.9-044744  &   194.7      &   -4.79583   &     0.586?  &  1.93$\pm$0.11  &   2.50$\pm$0.62   &   61.2 &  2.64$^{+1.10}_{-0.87}$   & 13.5$^{+4.7}_{-3.2}$ \\ 
  1BIGBJ130145.6+405623  &   195.44     &   40.94      &     0.652   &  2.18$\pm$0.15  &   2.04$\pm$0.40   &   71.5 &  1.71$^{+0.63}_{-0.49}$   &  6.3$^{+2.3}_{-1.5}$ \\ 
  1BIGBJ130713.3-034430  &   196.80542  &   -3.74194   &     0.      &  2.05$\pm$0.26  &   1.14$\pm$0.57   &   19.0 &  1.08$^{+1.03}_{-0.64}$   &  4.7$^{+4.2}_{-1.9}$ \\ 
  1BIGBJ132541.8-022809  &   201.42417  &   -2.46944   &     0.8?    &  1.93$\pm$0.18  &   1.13$\pm$0.42   &   27.3 &  1.19$^{+0.80}_{-0.56}$   &  6.0$^{+3.6}_{-2.0}$ \\ 
  1BIGBJ132617.7+122957  &   201.57375  &   12.49944   &     0.204   &  2.08$\pm$0.20  &   1.57$\pm$0.50   &   32.2 &  1.44$^{+0.87}_{-0.61}$   &  6.0$^{+3.6}_{-1.9}$ \\ 
  1BIGBJ132833.4+114520  &   202.13958  &   11.75556   &     0.811   &  1.92$\pm$0.17  &   1.31$\pm$0.46   &   37.5 &  1.40$^{+0.90}_{-0.63}$   &  7.1$^{+4.1}_{-2.3}$ \\ 
  1BIGBJ133612.1+231958  &   204.05042  &   23.33278   &     0.267   &  1.97$\pm$0.15  &   1.66$\pm$0.42   &   62.5 &  1.68$^{+0.79}_{-0.59}$   &  8.0$^{+3.6}_{-2.3}$ \\ 
  1BIGBJ135328.0+560056  &   208.36667  &   56.01556   &     0.404   &  2.25$\pm$0.15  &   2.13$\pm$0.42   &   71.0 &  1.69$^{+0.61}_{-0.48}$   &  5.7$^{+2.0}_{-1.3}$ \\ 
  1BIGBJ140629.9-393508  &   211.625    &   -39.58583  &     0.37    &  1.54$\pm$0.16  &   0.56$\pm$0.27   &   42.7 &  0.96$^{+0.87}_{-0.56}$   &  9.0$^{+5.9}_{-3.3}$ \\ 
  1BIGBJ143342.7-730437  &   218.42792  &   -73.07722  &     0.      &  1.33$\pm$0.20  &   0.15$\pm$0.11   &   24.6 &  0.36$^{+0.55}_{-0.29}$   &  4.7$^{+4.6}_{-2.2}$ \\ 
  1BIGBJ143825.4+120418  &   219.60625  &   12.07167   &     0.      &  2.11$\pm$0.21  &   1.35$\pm$0.49   &   25.2 &  1.20$^{+0.82}_{-0.56}$   &  4.8$^{+3.1}_{-1.6}$ \\ 
  1BIGBJ144236.4-462300  &   220.65167  &   -46.38361  &     0.103   &  1.92$\pm$0.10  &   3.14$\pm$0.64   &  107.7 &  3.33$^{+1.14}_{-0.93}$   & 17.1$^{+5.0}_{-3.6}$ \\ 
  1BIGBJ145543.6-760051  &   223.93167  &   -76.01444  &     0.      &  1.61$\pm$0.12  &   0.63$\pm$0.22   &   43.7 &  0.96$^{+0.59}_{-0.43}$   &  7.9$^{+3.6}_{-2.3}$ \\ 
  1BIGBJ145603.5+504825  &   224.015    &   50.80722   &  $>$0.49    &  2.09$\pm$0.24  &   1.23$\pm$0.55   &   27.2 &  1.11$^{+0.92}_{-0.60}$   &  4.5$^{+3.4}_{-1.6}$ \\ 
  1BIGBJ150637.0-054004  &   226.65458  &   -5.66778   &     0.518   &  1.72$\pm$0.17  &   0.94$\pm$0.41   &   35.2 &  1.25$^{+1.00}_{-0.67}$   &  8.7$^{+5.5}_{-3.1}$ \\ 
  1BIGBJ151041.0+333503  &   227.67125  &   33.58444   &     0.114   &  1.59$\pm$0.30  &   0.27$\pm$0.24   &   15.2 &  0.43$^{+0.91}_{-0.40}$   &  3.7$^{+6.4}_{-2.1}$ \\ 
  1BIGBJ151136.8-165326  &   227.90375  &   -16.89056  &  $>$0.56    &  2.15$\pm$0.35  &   1.22$\pm$0.74   &   13.1 &  1.06$^{+1.36}_{-0.74}$   &  4.0$^{+5.3}_{-1.8}$ \\ 
  1BIGBJ151618.7-152344  &   229.07792  &   -15.39556  &  $>$0.54    &  1.98$\pm$0.18  &   1.50$\pm$0.58   &   27.2 &  1.51$^{+1.02}_{-0.72}$   &  7.1$^{+4.1}_{-2.3}$ \\ 
  1BIGBJ151826.5+075222  &   229.61083  &   7.87278    &     0.41    &  1.74$\pm$0.20  &   0.66$\pm$0.33   &   24.6 &  0.85$^{+0.81}_{-0.51}$   &  5.7$^{+4.5}_{-2.3}$ \\ 
  1BIGBJ151845.7+061355  &   229.69042  &   6.23222    &     0.102   &  1.96$\pm$0.21  &   1.36$\pm$0.56   &   31.8 &  1.39$^{+1.09}_{-0.72}$   &  6.8$^{+5.0}_{-2.5}$ \\ 
  1BIGBJ152646.6-153025  &   231.69417  &   -15.50722  &  $>$0.43    &  2.04$\pm$0.13  &   2.61$\pm$0.64   &   58.4 &  2.47$^{+1.06}_{-0.82}$   & 10.8$^{+4.1}_{-2.7}$ \\ 
  1BIGBJ152913.5+381216  &   232.30625  &   38.20472   &  $>$0.59    &  2.04$\pm$0.19  &   1.22$\pm$0.39   &   34.6 &  1.16$^{+0.69}_{-0.49}$   &  5.1$^{+2.9}_{-1.6}$ \\ 
  1BIGBJ154202.9-291509  &   235.5125   &   -29.2525   &     0.      &  1.78$\pm$0.08  &   2.62$\pm$0.50   &  143.2 &  3.27$^{+1.04}_{-0.86}$   & 20.8$^{+5.4}_{-4.1}$ \\ 
  1BIGBJ154625.0-285723  &   236.60417  &   -28.95639  &  $>$0.6     &  1.73$\pm$0.18  &   0.67$\pm$0.36   &   18.7 &  0.88$^{+0.84}_{-0.54}$   &  6.0$^{+4.3}_{-2.3}$ \\ 
  1BIGBJ155053.2-082245  &   237.72167  &   -8.37944   &     0.      &  1.87$\pm$0.14  &   1.96$\pm$0.63   &   64.9 &  2.20$^{+1.24}_{-0.91}$   & 12.2$^{+5.8}_{-3.6}$ \\ 
  1BIGBJ155432.5-121324  &   238.63542  &   -12.22361  &     0.      &  1.69$\pm$0.13  &   1.04$\pm$0.39   &   34.3 &  1.45$^{+0.94}_{-0.68}$   & 10.6$^{+5.3}_{-3.3}$ \\ 
  1BIGBJ160218.0+305108  &   240.575    &   30.8525    &  $>$0.47    &  2.44$\pm$0.27  &   1.83$\pm$0.47   &   33.8 &  1.27$^{+0.70}_{-0.48}$   &  3.6$^{+2.3}_{-1.1}$ \\ 
  1BIGBJ160519.0+542058  &   241.32917  &   54.34972   &     0.212   &  1.88$\pm$0.13  &   1.13$\pm$0.29   &   64.0 &  1.25$^{+0.59}_{-0.45}$   &  6.8$^{+3.0}_{-1.9}$ \\ 
  1BIGBJ160618.4+134532  &   241.57667  &   13.75889   &     0.29    &  2.05$\pm$0.21  &   1.76$\pm$0.64   &   33.8 &  1.65$^{+1.14}_{-0.77}$   &  7.1$^{+4.7}_{-2.5}$ \\ 
  1BIGBJ161327.1-190835  &   243.36292  &   -19.14333  &     0.      &  2.14$\pm$0.15  &   3.15$\pm$0.82   &   34.1 &  2.73$^{+1.25}_{-0.95}$   & 10.5$^{+4.3}_{-2.7}$ \\ 
  1BIGBJ162115.1-003140  &   245.31333  &   -0.52778   &  $>$0.52    &  1.80$\pm$0.21  &   0.77$\pm$0.41   &   14.4 &  0.93$^{+0.93}_{-0.58}$   &  5.6$^{+4.7}_{-2.3}$ \\ 
  1BIGBJ162330.4+085724  &   245.87708  &   8.95667    &     0.533   &  1.91$\pm$0.20  &   1.23$\pm$0.52   &   35.5 &  1.33$^{+1.05}_{-0.69}$   &  7.0$^{+4.9}_{-2.5}$ \\ 
  1BIGBJ162646.0+630047  &   246.69167  &   63.01333   &     0.      &  1.91$\pm$0.17  &   1.00$\pm$0.33   &   51.6 &  1.07$^{+0.65}_{-0.46}$   &  5.5$^{+3.1}_{-1.8}$ \\ 
  1BIGBJ164220.2+221143  &   250.58458  &   22.19528   &     0.592   &  2.19$\pm$0.19  &   1.76$\pm$0.55   &   32.1 &  1.46$^{+0.83}_{-0.60}$   &  5.3$^{+2.8}_{-1.6}$ \\ 
  1BIGBJ164419.9+454644  &   251.08333  &   45.77889   &     0.225   &  1.65$\pm$0.16  &   0.48$\pm$0.20   &   39.1 &  0.70$^{+0.56}_{-0.37}$   &  5.4$^{+3.5}_{-2.0}$ \\ 
  1BIGBJ165517.8-224045  &   253.82458  &   -22.67917  &     0.      &  1.99$\pm$0.21  &   1.64$\pm$0.75   &   17.4 &  1.64$^{+1.38}_{-0.91}$   &  7.7$^{+5.6}_{-2.8}$ \\ 
  1BIGBJ171108.5+024403  &   257.78583  &   2.73444    &     0.      &  1.83$\pm$0.18  &   0.93$\pm$0.42   &   18.3 &  1.09$^{+0.89}_{-0.60}$   &  6.4$^{+4.2}_{-2.3}$ \\ 
  1BIGBJ174419.7+185218  &   266.0825   &   18.87167   &     0.      &  1.58$\pm$0.21  &   0.41$\pm$0.26   &   15.5 &  0.65$^{+0.85}_{-0.48}$   &  5.7$^{+5.6}_{-2.6}$ \\ 
  1BIGBJ174702.5+493800  &   266.76042  &   49.63361   &     0.46?   &  2.27$\pm$0.22  &   1.74$\pm$0.49   &   37.3 &  1.37$^{+0.75}_{-0.53}$   &  4.5$^{+2.6}_{-1.4}$ \\ 
  1BIGBJ184822.4+653656  &   282.09375  &   65.61583   &     0.364   &  1.59$\pm$0.15  &   0.50$\pm$0.21   &   52.8 &  0.79$^{+0.63}_{-0.42}$   &  6.8$^{+4.2}_{-2.4}$ \\ 
  1BIGBJ185023.9+263153  &   282.6      &   26.53139   &     0.      &  1.63$\pm$0.13  &   1.20$\pm$0.45   &   88.6 &  1.80$^{+1.18}_{-0.85}$   & 14.5$^{+7.1}_{-4.5}$ \\ 
  1BIGBJ185813.3+432451  &   284.55583  &   43.41417   &     0.      &  2.12$\pm$0.16  &   1.89$\pm$0.48   &   43.3 &  1.67$^{+0.77}_{-0.58}$   &  6.6$^{+2.9}_{-1.8}$ \\ 
  1BIGBJ193412.7-241919  &   293.55292  &   -24.32222  &     0.      &  1.60$\pm$0.12  &   0.88$\pm$0.30   &   53.5 &  1.36$^{+0.81}_{-0.59}$   & 11.5$^{+5.2}_{-3.4}$ \\ 
  1BIGBJ194356.2+211821  &   295.98417  &   21.30611   &     0.      &  1.44$\pm$0.08  &   2.01$\pm$0.57   &  194.7 &  3.93$^{+1.84}_{-1.44}$   & 42.9$^{+13.2}_{-9.8}$ \\   
  1BIGBJ200204.0-573644  &   300.51708  &   -57.6125   &     0.      &  2.08$\pm$0.10  &   2.93$\pm$0.49   &  105.5 &  2.69$^{+0.78}_{-0.64}$   & 11.2$^{+3.0}_{-2.2}$ \\ 
  1BIGBJ201200.9-771219  &   303.00375  &   -77.20528  &     0.      &  2.10$\pm$0.30  &   0.78$\pm$0.52   &    9.8 &  0.71$^{+0.89}_{-0.52}$   &  2.8$^{+3.0}_{-1.2}$ \\ 
  1BIGBJ205242.4+081040  &   313.17708  &   8.17778    &     0.      &  1.51$\pm$0.23  &   0.25$\pm$0.20   &   15.3 &  0.45$^{+0.73}_{-0.37}$   &  4.3$^{+5.1}_{-2.2}$ \\ 
  1BIGBJ214533.3-043438  &   326.38875  &   -4.5775    &     0.069   &  2.64$\pm$0.31  &   1.34$\pm$0.47   &    9.7 &  0.82$^{+0.55}_{-0.37}$   &  1.9$^{+1.2}_{-0.6}$ \\ 
  1BIGBJ215214.0-120540  &   328.05875  &   -12.09472  &     0.121   &  2.26$\pm$0.14  &   3.77$\pm$0.76   &   81.3 &  2.98$^{+1.06}_{-0.84}$   & 10.0$^{+3.3}_{-2.2}$ \\ 
  1BIGBJ220107.3-590639  &   330.28042  &   -59.11111  &     0.      &  1.93$\pm$0.18  &   0.78$\pm$0.28   &   21.3 &  0.82$^{+0.55}_{-0.38}$   &  4.1$^{+2.4}_{-1.4}$ \\ 
  1BIGBJ220155.8-170700  &   330.4825   &   -17.11667  &     0.169   &  1.32$\pm$0.37  &   0.16$\pm$0.22   &   33.5 &  0.38$^{+1.63}_{-0.47}$   &  5.1$^{+14.1}_{-3.5}$ \\  
  1BIGBJ221029.5+362159  &   332.62333  &   36.36639   &     0.      &  2.17$\pm$0.32  &   1.19$\pm$0.75   &   13.3 &  1.01$^{+1.23}_{-0.72}$   &  3.7$^{+4.1}_{-1.6}$ \\ 
  1BIGBJ221108.2-000302  &   332.78458  &   -0.05056   &     0.326   &  1.84$\pm$0.14  &   1.43$\pm$0.47   &   48.7 &  1.67$^{+0.98}_{-0.71}$   &  9.7$^{+4.8}_{-2.9}$ \\ 
  1BIGBJ223301.0+133601  &   338.25458  &   13.60028   &     0.214   &  1.51$\pm$0.24  &   0.24$\pm$0.19   &   15.4 &  0.43$^{+0.73}_{-0.37}$   &  4.2$^{+5.1}_{-2.1}$ \\ 
  1BIGBJ223626.2+370713  &   339.10958  &   37.12028   &     0.      &  1.85$\pm$0.20  &   0.98$\pm$0.48   &   29.1 &  1.12$^{+1.01}_{-0.66}$   &  6.3$^{+4.8}_{-2.4}$ \\ 
  1BIGBJ224910.6-130002  &   342.29458  &   -13.00056  &  $>$0.5     &  2.33$\pm$0.01  &  87.01$\pm$1.43   &11240.5 &  64.8$^{+1.93}_{-1.88}$   &202.8$^{+6.2}_{-6.0}$ \\ 
  1BIGBJ225147.5-320611  &   342.94792  &   -32.10333  &     0.246   &  2.07$\pm$0.19  &   1.60$\pm$0.51   &   48.6 &  1.48$^{+0.90}_{-0.63}$   &  6.2$^{+3.7}_{-2.0}$ \\ 
  1BIGBJ225613.3-330338  &   344.05542  &   -33.06056  &     0.243   &  2.56$\pm$0.21  &   2.23$\pm$0.42   &   39.7 &  1.42$^{+0.54}_{-0.41}$   &  3.6$^{+1.4}_{-0.8}$ \\  
  1BIGBJ230634.9-110347  &   346.64583  &   -11.06333  &     0.      &  1.69$\pm$0.21  &   0.62$\pm$0.34   &   28.5 &  0.86$^{+0.94}_{-0.56}$   &  6.3$^{+5.7}_{-2.7}$ \\ 
  1BIGBJ232039.7-630918  &   350.16583  &   -63.155    &     0.2     &  1.84$\pm$0.16  &   0.84$\pm$0.30   &   43.6 &  0.98$^{+0.64}_{-0.45}$   &  5.7$^{+3.2}_{-1.8}$ \\ 
  1BIGBJ233112.8-030129  &   352.80375  &   -3.025     &     0.      &  2.05$\pm$0.15  &   1.95$\pm$0.54   &   40.8 &  1.84$^{+0.90}_{-0.67}$   &  7.9$^{+3.5}_{-2.2}$ \\ 
  1BIGBJ235320.9-145856  &   358.3375   &   -14.9825   &     0.      &  1.83$\pm$0.28  &   0.55$\pm$0.37   &   13.3 &  0.65$^{+0.92}_{-0.49}$   &  3.8$^{+4.9}_{-1.9}$ \\ 
 \hline
 \end{tabular}
\end{table*}
